DFormer: Rethinking RGBD Representation Learning for Semantic Segmentation

We present DFormer, a novel RGB-D pretraining framework to learn transferable representations for RGB-D segmentation tasks. DFormer has two new key innovations: 1) Unlike previous works that encode RGB-D information with RGB pretrained backbone, we pretrain the backbone using image-depth pairs from ImageNet-1K, and hence the DFormer is endowed with the capacity to encode RGB-D representations; 2) DFormer comprises a sequence of RGB-D blocks, which are tailored for encoding both RGB and depth information through a novel building block design. DFormer avoids the mismatched encoding of the 3D geometry relationships in depth maps by RGB pretrained backbones, which widely lies in existing methods but has not been resolved. We finetune the pretrained DFormer on two popular RGB-D tasks, i.e., RGB-D semantic segmentation and RGB-D salient object detection, with a lightweight decoder head. Experimental results show that our DFormer achieves new state-of-the-art performance on these two tasks with less than half of the computational cost of the current best methods on two RGB-D semantic segmentation datasets and five RGB-D salient object detection datasets. Our code is available at: https://github.com/VCIP-RGBD/DFormer.

==> tables/ablation.tex <==
\begin{subtable}[t]{0.95\textwidth}
	\begin{center}
    	\caption{\small Accuracy, parameters, flops as a function of the model size on the three datasets. 
        ``SS'' and ``MS'' means single/multi-scale test.}
        \vspace{-4pt}
        \footnotesize
        \begin{tabular}{c|c c|cc|cc|cc}
            % \toprule
            % \multicolumn{9}{c}{SegFormer}\\
            \toprule
            Encoder  & \multicolumn{2}{c|}{Params} & \multicolumn{2}{c|}{NYUDepthv2~\cite{}} & \multicolumn{2}{c|}{SUN-RGBD~\cite{}} & \multicolumn{2}{c}{DELIVER~\cite{}} \\ \cline{2-9} 
             Model   & Encoder &Decoder & Flops $\downarrow$  & mIoU(SS/MS) $\uparrow$  & Flops $\downarrow$  & mIoU(SS/MS) $\uparrow$  & Flops $\downarrow$  & mIoU(SS)  $\uparrow$ \\ \midrule
             \nameofmethod{}-T & 3.4  &0.4& 8.4 & 37.4~/~38.0 & 125.5 & 76.2~/~78.1 & 8.4 & 35.6 \\ %\cline{2-9} 
             \nameofmethod{}-S & 13.1 &0.6& 15.9 & 42.2~/~43.1 & 243.7 & 78.5~/~80.0 & 15.9 & 40.2 \\ %\cline{2-9} 
             \nameofmethod{}-B & 24.2 &3.3& 62.4 & 46.5~/~47.5 & 717.1 & 81.0~/~82.2 & 62.4 & 44.6 \\ %\cline{2-9} 
             \nameofmethod{}-L & 44.0 &3.3& 79.0 & 49.4~/~50.0 & 962.9 & 81.7~/~83.3 & 79.0 & 45.5 \\ %\cline{2-9} 
             \bottomrule
        \end{tabular}
	\label{tab:modelsize}
	\end{center}
\end{subtable}
\vspace{5mm}
% MLP DIM
\begin{subtable}[ht]{0.59\textwidth}
        \footnotesize
	\begin{center}
 \vspace{3pt}
    \caption{\small RGB-D pretraining pipeline. `Baseline' is composed of the base block.}
    \label{tab:ablation_ppl}
    \vspace{-5pt}
    \footnotesize
    \setlength\tabcolsep{5pt}
        \begin{tabular}{l|cccc}
    \toprule
    \textbf{Model} &Pretrain& \textbf{\#Params}  & \textbf{FLOPs} & \textbf{mIoU (\%)} \\
    \midrule\midrule
    Baseline&RGB& 66.6 & 67.6 &  \\
    Baseline&RGB+Depth& 66.7 & 67.6 &  \\
    \nameofmethod{}-B &RGB& 139.9 & 134.3 &  \\
    \nameofmethod{}-B &RGB+Depth& 28.5 & 41.8 & 55.1\\
    \bottomrule
\end{tabular}
	    \label{tab:ppl}
	\end{center}
\end{subtable}
% \hspace{5pt}
\hspace{2pt}
\begin{subtable}[ht]{0.39\textwidth}
        \footnotesize
	\begin{center}
  \vspace{3pt}
    \caption{\small Componets in our RGB-D block. }
    \label{tab:ab_block}
    \vspace{-5pt}
    \footnotesize
    \setlength\tabcolsep{5pt}
        \begin{tabular}{ll|ccc}
    \toprule
    \textbf{LSE} &\textbf{CMA}& \textbf{\#Params}  & \textbf{FLOPs} & \textbf{mIoU (\%)} \\
    \midrule\midrule
    \usym{2718}&\usym{2718}& 66.6 & 67.6 &  \\
    \usym{2714}&\usym{2718}& 66.7 & 67.6 &  \\
    \usym{2718}&\usym{2714}&\\
    \usym{2714}&\usym{2714}& 28.5 & 41.8 &55.1  \\
    \bottomrule
\end{tabular}
	\end{center}
\end{subtable}
% 
% \vspace{5mm}
\hspace{2pt}
\begin{subtable}[ht]{0.46\textwidth}
	\footnotesize
	\begin{center}
    \caption{\small Input of classification layer for \nameofmethod{}-B during pretraining. `$X_{RGB}^{l}$' and `$X_{D}^{l}$' respectively mean the RGB and Depth features generated by the last stage.}
    \label{tab:ablation_ppl}
    \vspace{5pt}
    \footnotesize
    \setlength\tabcolsep{5pt}
        \begin{tabular}{l|ccc}
    \toprule
    Feature& \textbf{\#Params}  & \textbf{FLOPs} & \textbf{mIoU (\%)} \\
    \midrule\midrule
    $X_{RGB}^{l}$& 66.6 & \textbf{67.6} & 54.1 \\
    $X_{RGB}^{l}+X_{D}^{l}$& 181.1 & 167.8 & \textbf{56.8} \\
    \bottomrule
\end{tabular}
	    \label{tab:ab_prelayer}
	\end{center}
\end{subtable}
% \hspace{5pt}
\hspace{2pt}
\begin{subtable}[ht]{0.46\textwidth}
	\footnotesize
    \caption{\small Input of the decoder head for \nameofmethod{}-B during finetuning. `$X_{RGB}$+$X_{D}$' means simultaneously uses features from RGB and depth parts as the input of the decoder head.   }
    \label{tab:ab_head}
    \vspace{5pt}
    \footnotesize
    \centering
    \setlength\tabcolsep{5pt}
        \begin{tabular}{l|ccc}
    \toprule
    Feature& \textbf{\#Params}  & \textbf{FLOPs} & \textbf{mIoU (\%)} \\
    \midrule\midrule
    $X_{RGB}$ (\textbf{Ours})& 66.6 & \textbf{67.6} & 54.1 \\
    $X_{RGB}+X_{D}$& 181.1 & 167.8 & \textbf{56.8} \\
    \bottomrule
\end{tabular}
\end{subtable}
\vspace{10pt}


==> tables/gfl_test.tex <==
% %Results of SegFormer-B0 to B5 on ADE20K, Cityscapes validation set and COCO-Stuff full dataset
%Results of SegFormer-B0 to B5 on ADE20K, Cityscapes validation set and COCO-Stuff full dataset
\begin{subtable}[ht]{0.45\textwidth}
	\begin{center}
		\captionsetup{font={scriptsize}}
	    \caption{Accuracy as a function of the MLP dimension $C$ in the decoder on ADE20K.}
	    \vspace{-4pt}
		\setlength{\tabcolsep}{2mm}
		\resizebox{\textwidth}{!}{
		 \begin{tabular}{l|cc}
    \toprule
    \textbf{Pre-train Manner} & Input& \textbf{mIoU (\%)} \\
    \midrule\midrule
    % \# 1&Baseline&RGB&  &  &  \\
    % \# 1&Dual Baseline&RGB& 53M  & 61.2G &  \\
    RGB&RGB+RGB & 53.3 \\
    \nameofmethod{} (Ours)&RGB+Depth& 55.6\\
    \bottomrule
\end{tabular}
		}
	    \label{tab:mlpdim}
	\end{center}
\end{subtable}
% \hspace{5pt}
\hspace{2pt}
\begin{subtable}[ht]{0.45\textwidth}
	\begin{center}
		\captionsetup{font={scriptsize}}
		\caption{Mix-FFN vs. positional encoding (PE) for different test resolution on Cityscapes.}
		%\caption{Accuracy as a function of using Mix-FFN or a positional encoding (PE) for different test resolution on Cityscapes. For training we used 768$\times$768 image crops.}
		\vspace{-4pt}
		\setlength{\tabcolsep}{2mm}
		\resizebox{\textwidth}{!}{
    		\begin{tabular}{l|ccc}
    \toprule
    Decoder input& \textbf{\#Params}  & \textbf{FLOPs} & \textbf{mIoU}\textbf{(SS/MS)} \\
    \midrule\midrule
    $X_{RGB}$ (\textbf{Ours})& 66.6 & \textbf{67.6} & 55.3/55.6 \\
    $X_{RGB}+X_{D}$& 67.2 & 69.8 & 55.1/55.4 \\
    \bottomrule
\end{tabular}
		}
		\label{tab:resolution}
	\end{center}
\end{subtable}
% 


==> tables/main_table.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \caption{Comparison with state-of-the-art methods on the ADE20K, Cityscapes and COCO-Stuff benchmarks. The number of FLOPs (G) is calculated on the input size of 512$\times$512 for ADE20K and COCO-Stuff, and 2,048$\times$1,024 for Cityscapes. $^{\dagger}$ means models pretrained on ImageNet-22K.}
    \begin{tabular}{lccccccccc} \toprule
    \multirow{2}{*}{Model}  & Params & \multicolumn{4}{c}{ADE20K} & \multicolumn{4}{c}{Cityscapes}  \\ \cmidrule(lr){3-6}\cmidrule(lr){7-10}
    & (M) & Input Size & GFLOPs  & mIoU (SS) & mIoU (MS)  & Input Size & GFLOPs  & mIoU (SS) & mIoU (MS) \\ \midrule
     Segformer-B0~\cite{xie2021segformer}  & 3.8 & $512\times512$ & 8.4 & 37.4 & 38.0 & $1024\times2048$ & 125.5 & 76.2 & 78.1 \\ 
     SegNeXt-T~\cite{guo2022segnext} & 4.3 & $512\times512$ & 6.6 & 41.1 & 42.2 & $1024\times2048$ & 50.5 & 79.8 & 81.4  \\  
     \nameofmethod{}-T & 4.3 & $512\times512$ & 5.9 & 42.1 & - & $1024\times2048$ & - & - & - \\ \midrule
    Segformer-B1~\cite{xie2021segformer} & 13.7 & $512\times512$ & 15.9 & 42.2 & 43.1 & $1024\times2048$ & 243.7 & 78.5 & 80.0 \\  
     HRFormer-S~\cite{yuan2021hrformer} & 13.5 & $512\times512$ & 109.5 & 44.0 & 45.1 & $1024\times2048$ & 835.7 & 80.0 & 81.0 \\ 
     SegNeXt-S~\cite{guo2022segnext} & 13.9 & $512\times512$ & 15.9 & 44.3 & 45.8 & $1024\times2048$ & 124.6 & 81.3 & 82.7  \\ 
      \nameofmethod{}-S & 14.0 & $512\times512$ & 15.1 & 45.0 & - & $1024\times2048$ & - & - & - \\ \midrule
     Segformer-B2~\cite{xie2021segformer}  & 27.5 & $512\times512$ & 62.4 & 46.5 & 47.5 & $1024\times2048$ & 717.1 & 81.0 & 82.2 \\
     MaskFormer~\cite{cheng2021maskformer} & 42 & $512\times512$ & 55 & 46.7 & 48.8 & $1024\times2048$ & - & - & -  \\ 
     SegNeXt-B~\cite{guo2022segnext} & 27.6 & $512\times512$ & 34.9 & 48.5 & 49.9 & $1024\times2048$ & 275.7 & 82.6 & 83.8 \\ 
      \nameofmethod{}-B & - & $512\times512$ & - & - & - & $1024\times2048$ & - & - & - \\ \midrule
     SETR-MLA$^{\dagger}$\cite{zheng2021rethinking} & 310.6 & $512\times512$ & - & 48.6 & 50.1 & $1024\times2048$ & - & 79.3 & 82.2 \\  
     DPT-Hybrid~\cite{ranftl2021vision} & 124.0 & $512\times512$ & 307.9 & - & 49.0 & $1024\times2048$ & - & - & - \\
     Segformer-B3~\cite{xie2021segformer} & 47.3 & $512\times512$ & 79.0 & 49.4 & 50.0 & $1024\times2048$ & 962.9 & 81.7 & 83.3 \\  
    %  Segformer-B4~\cite{xie2021segformer} & 64.1 & 95.7 & 50.3 & 51.1 & 1240.6 & 82.3 & 83.9 & 95.7 & \textbf{46.5} & - \\ 
     Mask2Former~\cite{cheng2021mask2former} & 47 & $512\times512$ & 74 & 47.7 & 49.6 & $1024\times2048$ & - & - & - \\ 
     HRFormer-B~\cite{yuan2021hrformer} & 56.2 & $512\times512$ & 280.0 & 48.7 & 50.0 & $1024\times2048$ & 2223.8 & 81.9 & 82.6  \\ 
     MaskFormer~\cite{cheng2021maskformer} & 63 & $512\times512$ & 79 & 49.8 & 51.0 & $1024\times2048$ & - & -   \\ 
     SegNeXt-L~\cite{guo2022segnext}  & 48.9 & $512\times512$ & 70.0 & 51.0 & 52.1 & $1024\times2048$ & 577.5 & 83.2 & 83.9 \\  
      \nameofmethod{}-L  & - & $512\times512$ & - & - & - & $1024\times2048$ & - & - & - \\  \bottomrule
    \end{tabular}
    \label{tab:ade20k_city_stuff}
\end{table*}

==> tables/rgbd_seg_nocite.tex <==
% \newcommand{\nameofmethod}{DepthNext}
\begin{table}[tp]
  \centering
% \vskip -1ex
    % \setlength\tabcolsep{6pt}
    % \vskip -1ex
    \setlength{\tabcolsep}{3.5pt}
    \scriptsize
    \caption{\small Results on NYU Depth V2~\citep{silberman2012nyu_dataset} and SUN-RGBD~\citep{song2015sun_rgbd} datasets. `$^{*}$' denote single-scale test. `$^{\dag}$' indicates our implemented results.}
    \centering
    \renewcommand{\arraystretch}{0.9}
    	\begin{tabular}{lccccccccc}
        \toprule
        \textbf{\multirow{2}{*}{Model}}  &\textbf{\multirow{2}{*}{Backbone}}   & \textbf{\multirow{2}{*}{Params}} &\multicolumn{3}{c}{NYUDepthv2} & \multicolumn{3}{c}{SUN-RGBD} &\textbf{\multirow{2}{*}{Code}}\\ \cmidrule(lr){4-6}\cmidrule(lr){7-9}
         && &\textbf{Input size}& \textbf{Flops}& \textbf{mIoU}   &\textbf{Input size}& \textbf{Flops}& \textbf{mIoU} & \\
        \midrule\midrule
        %FCN~\cite{long2015fcn} & 29.2 & 49.2 \\
        % 3DGNN$_{\rm ICCV2017*}$~\cite{qi20173d} &&&$480\times 640$&& 43.1 & - &&&45.9&-\\
        % Kong $et\ al.$~\cite{kong2018recurrent}&&&$480\times 640$ && 44.5 & 72.1 \\
        % LS-DeconvNet$_{2017}$~\cite{cheng2017locality}&&&$480\times 640$ && 45.9 & 71.9\\
        % CFN$_{\rm ICCV2017}$~\cite{CaRF17}&&&$480\times 640$ && 47.7 & -&&&48.1&- \\
        ACNet$_{\rm 19*}$&ResNet-50&116.6M&$480\times 640$ &126.7G& 48.3 &$530\times 730$&163.9G&48.1&\href{https://github.com/anheidelonghu/ACNet}{Link} \\
        PSD$_{\rm 20*}$&ResNet-50&&$480\times 640$ &&51.0&&&50.6&N/A\\
        CANet$_{\rm 20*}$&ResNet-101&&$480\times 640$&&51.2&&&48.3&N/A\\
        % RDF$_{\rm ICCV2017*}$~\cite{park2017rdfnet}&&ResNet-101&$480\times 640$ && 49.1 & 75.6&&&&\\
        SGNet$_{\rm 20*}$&ResNet-101&64.7M&$480\times 640$ && 51.1 &&&48.6&\href{https://github.com/LinZhuoChen/SGNet}{Link}\\
        \rowcolor{gray!15} ESANet$_{\rm 21}$&ResNet-34&31.2M&$480\times 640$&34.9G&50.3&$480\times 640$&34.9G&48.2&\href{https://github.com/TUI-NICR/ESANet}{Link}\\
        GLPNet$_{\rm 21}$&ResNet-101&&&&54.6&&&51.2&N/A\\
        FSFNet$_{\rm 21*}$&&&&&52.0&&&50.6&N/A\\
        NANet$_{\rm 21}$&&&$480\times 640$& & 52.3 &&&48.8&N/A \\
        PGDENet$_{\rm 22}$&ResNet-34&100.7M&$480\times 640$&178.8G&53.7&$530\times730$&229.1G&51.0&\href{https://github.com/EnquanYang2022/PGDENet}{Link}\\
        SA-Gate$_{\rm 20*}$&ResNet-101&110.9M&$480\times 640$ &193.7G& 52.4 &$530\times 730$&250.1G&49.4&\href{https://github.com/charlesCXK/RGBD_Semantic_Segmentation_PyTorch}{Link} \\
        DCANet$_{\rm 22*}$&ResNet-101&&&&53.3&&&49.6&N/A\\
        WTNet$_{\rm 22}$&&&&&52.1&&&50.2&N/A\\
        FAFNet$_{\rm 23}$&&&&&54.0&&&49.2&N/A\\
        MGCNet$_{\rm 22}$&&&&&54.5&&&51.5&N/A\\
        FRNet$_{\rm 22}$&ResNet-34&85.5M&$480\times 640$&115.6G&53.6&$530\times 730$&150.0G&51.8&\href{https://github.com/EnquanYang2022/FRNet}{Link}\\
        RFNet$_{\rm 22}$&&&&&53.5&&&50.7&N/A\\ \midrule
        % ZigZagNet$_{\rm 20}$~\cite{}
        ShapeConv$_{\rm 21*}$&ResNext-101&&$480\times 640$ && 51.3 &$530\times 730$&&48.6&\href{https://github.com/hanchaoleng/ShapeConv}{Link} \\ %&62.6 f. w. mIoU
        CEN$_{\rm 20}$&ResNet-101&118.2M&$480\times 640$&618.7G&51.1$^{*}$/51.7&$530\times 730$&790.3G&49.6/50.2&\href{https://github.com/yikaiw/CEN}{Link}\\
        CEN$_{\rm 20}$&ResNet-152&133.9M&$480\times 640$&664.4G&52.5&$530\times 730$&849.7G&51.1&\href{https://github.com/yikaiw/CEN}{Link}\\
        \rowcolor{gray!15} EMSANet$_{\rm 22}$&ResNet-34&46.9M&$480\times 640$&45.4G&51.0&$530\times 730$&58.6G&48.4&\href{https://github.com/TUI-NICR/EMSANet}{Link}\\ 
        TransD-Fusion$_{\rm 22}$&Swin-B&250.6M&&&55.5&&&51.9 &N/A\\
        \midrule
        TokenFusion$_{\rm 22*}$& MiT-B2&26.0M&$480\times640$&55.2G&53.3&&&&\href{https://github.com/yikaiw/TokenFusion}{Link}\\
        TokenFusion$_{\rm 22*}$ &MiT-B3&45.9M&$480\times640$&94.4G&54.2&&&&\href{https://github.com/yikaiw/TokenFusion}{Link}\\
        MultiMAE$_{\rm 22*}$&ViT-B&95.2M&$640\times640$&267.9G&56.0&$640\times 640$&267.9G&50.7$^{*\dag}$/52.0$^{\dag}$&\href{https://github.com/EPFL-VILAB/MultiMAE}{Link}\\
        Omnivore$_{\rm 22*}$&Swin-T&29.1M&$480\times 640$&32.7G&49.7&---&---&---&\href{https://github.com/facebookresearch/omnivore}{Link}\\
        Omnivore$_{\rm 22*}$&Swin-S&51.3M&$480\times 640$&59.8G&52.7&---&---&---&\href{https://github.com/facebookresearch/omnivore}{Link}\\
        Omnivore$_{\rm 22*}$&Swin-B&95.7M&$480\times 640$&109.3G&54.0&---&---&---&\href{https://github.com/facebookresearch/omnivore}{Link}\\
        CMX$_{\rm 22*}$&MiT-B2&66.6M&$480\times 640$&67.6G&54.1$^{*}$/54.4&$530\times730$&&49.7&\href{https://github.com/huaaaliu/RGBX_Semantic_Segmentation}{Link}\\
        CMX$_{\rm 22*}$&MiT-B4&139.9M&$480\times 640$&134.3G&56.0$^{*}$/56.3&$530\times730$&&52.1&\href{https://github.com/huaaaliu/RGBX_Semantic_Segmentation}{Link}\\
        CMX$_{\rm 22*}$&MiT-B5&181.1M&$480\times 640$&167.8G&56.8$^{*}$/56.9&$530\times730$&&52.4&\href{https://github.com/huaaaliu/RGBX_Semantic_Segmentation}{Link}\\
        CMNext$_{\rm 23}(\citeauthor{zhang2023delivering})$&MiT-B4&116.6M&$480\times640$&131.9G&/56.9&$530\times730$&170.3G&&\href{https://github.com/jamycheung/DELIVER}{Link}\\
        % \midrule
        % AMF$_{\rm 2022*}$&&ResNet-50&&&&&&49.6\\
        % PDCNet$_{\rm 2023*}$&&ResNet-101&&&&&&49.6\\
        % EMSAFormer$_{\rm 2023*}$&&&&&&&&48.8\\
        % EMSANet$_{\rm IJCNN2022*}$&&&&&53.3&&&48.5\\
        % LF$_{\rm 2023*}$&&Segformer-B2&&&&&&48.2\\
        % RedNet$_{\rm 2018*}$&&ResNet-50&&&&&&47.8\\
        % RDF-152$_{\rm ICCV2017*}$&&ResNet-152&&&50.1&&&47.7\\
        % CCL$_{\rm 2018*}$&&&&&&&&47.1\\
        % MMAF-Net-152$_{\rm 2019*}$&&&&&&&&47.0\\
        % UCTNet$_{\rm ECCV2022}$&&&&&57.6&&&&51.2&\\
        % CSNet$_{\rm JPRS2021}$&&&&&51.5&&&&52.8&\\
        % LWN$_{\rm TMM2021}$&&ResNet-152&&&51.5&&&&53.1&\\ %这个方法估计有问题
        \midrule
        \rowcolor{gray!15}\nameofmethod{}-T &Ours-T&6.0M&$480\times 640$& 11.8G&50.8&&&47.2/&\href{https://github.com/HVision-NKU}{Link} \\
        \rowcolor{gray!15}\nameofmethod{}-S &Ours-S&19.0M&$480\times 640$ &25.9G&53.1 &&&48.9/ &\href{https://github.com/HVision-NKU}{Link}\\
        \rowcolor{gray!15} \nameofmethod{}-B&Ours-B&29.5M&$480\times 640$ &41.9G&55.3$^{*}$/55.6&&&49.7$^{*}$/51.3&\href{https://github.com/HVision-NKU}{Link}\\
        \rowcolor{gray!15}\nameofmethod{}-L&Ours-L&&$480\times 640$ &&&&&&\href{https://github.com/HVision-NKU}{Link} \\
        \bottomrule
        \end{tabular}
    
    \hspace{\fill}
    \hspace{\fill}
    %=======================
    % \begin{subtable}[t]{0.99\columnwidth}
    % % \setlength\tabcolsep{6pt}
    % \footnotesize
    % \begin{subtable}[t]{\columnwidth}
    % \caption{Results on SUN-RGBD~\cite{song2015sun_rgbd}.}
    % \vskip -1ex
    % \label{tab:table_SUN}
    % \setlength{\tabcolsep}{5pt}  
    % \renewcommand{\arraystretch}{1.0}
    % 	\begin{tabular}{l|ccccc}
    %     \toprule
    %     \textbf{Method} &\textbf{Param}&\textbf{Input size} &\textbf{Flops}& \textbf{mIoU}  & \textbf{Acc}\\
    %     \midrule\midrule
    %     3DGNN~\cite{qi20173d} & &480$\times$480&&45.9  & - \\
    %     RDF-152~\cite{park2017rdfnet} & &480$\times$480&& 47.7 & 81.5 \\
    %     CFN~\cite{CaRF17}  & & 480$\times$480&&48.1 & - \\
    %     D-CNN~\cite{wang2018depth_aware}  & &480$\times$480&&42.0 & - \\
    %     ACNet~\cite{hu2019acnet} &  &480$\times$480&&48.1  & - \\
    %     %PAP~\cite{zhang2019pattern} & 50.5 & \textbf{83.8} \\
    %     TCD~\cite{yue2021two_stage} & &480$\times$480&& 49.5 & 83.1\\
    %     SGNet~\cite{chen2021spatial_guided}  & &480$\times$480&& 48.6  & 82.0 \\
    %     SA-Gate~\cite{chen2020sa_gate} & &480$\times$480&& 49.4  & 82.5 \\
    %     NANet~\cite{zhang2021non_aggregation} &  &480$\times$480&&48.8 & 82.3\\
    %     ShapeConv~\cite{cao2021shapeconv} & &480$\times$480&& 48.6  & 82.2\\
    %     PGDENet~\cite{}&100.6M&$480\times 640$&177.8G&51.0&\\
    %     CMX (MiT-B2)$^{*}$ &66.6 &480$\times$480& &49.7 & 82.8 \\ 
    %     CMX (MiT-B4)$^{*}$ &139.9&480$\times$480&& 52.1 & 83.5\\
    %     CMX (MiT-B5)$^{*}$ &181.1&480$\times$480&& \textbf{52.4} & \textbf{83.8}\\
    %     \midrule
    %     \nameofmethod{}-T &6.0M &480$\times$480&&47.2\\
    %     \nameofmethod{}-S & &480$\times$480&&48.7\\
    %     \nameofmethod{}-B & &480$\times$480\\
    %     \nameofmethod{}-L & &480$\times$480\\
    %     \bottomrule
    %     \end{tabular}
    
    % \end{subtable}%
    % \end{subtable}
    % \hspace{\fill}
    %=======================
\end{table}

==> tables/supp_SOD.tex <==
\begin{table}[t]
\scriptsize
\setlength\tabcolsep{2.2pt}
\setlength\extrarowheight{1pt}
\begin{center}
\caption{Quantitative comparisons on RGB-D SOD benchmarks. The best results are \highlight{highlighted}. `-' means the results of some methods are not provided in their paper.
% We use the Mean Absolute Error ($M$), max F-measure ($F$), S-measure ($S$), and max E-measure ($E$) as evaluation metrics.
}
\vspace{-10pt}
\label{tab:sod_supp}
% \resizebox{0.99\linewidth}{!}{
\begin{tabular}{lcc|| llll|llll|llll}
\toprule
 Dataset & Param  & Flops &\multicolumn{4}{c}{DUTLF-Depth}  & \multicolumn{4}{c}{ReDWeb-S}   & \multicolumn{4}{c}{LFSD}  \\%& \multicolumn{4}{c}{SSD} \\
\cline{4-7} \cline{8-11} \cline{12-15} %\cline{22-25}

Metric & \makecell{(M)} &\makecell{(G)}& $M$ &  $F$  &  $S$ &  $E$  &  $M$ &  $F $  &  $S$ &  $E$  &  $M$ &  $F $  &  $S$ &  $E$  \\%&  $M$ &  $F $  &  $S$ &  $E$\\
\hline
%$CPFP_{19}$ & .038 & .846 & .872  &.923 & .036 & .867 & .888  &.932 & .053 & .877 & .878  &.923 & .051 & .874 & .879  &.925 & .064 & .851 & .850  &.903 \\%& .082 & .766 & .807  &.852 \\


BBSNet$_{21}$ (\citeauthor{zhai2021bifurcated})& 49.8& 31.3&.058&.870&.882&.912&.150&.680&.693&.763&.092&.828&.835&.870 \\%& .044 & .859 & .882  &.919 \\

DCF$_{21}$ (\citeauthor{ji2021calibrated}) & 108.5& 54.3&.030&.926&.929&.952&-&-&-&-&-&-&-&-\\

DSA2F$_{21}$ (\citeauthor{sun2021deep})& 36.5 & 172.7 &.030&.926&.921&.950&-&-&-&- &.054&.882&.882&.923  \\%& .045 & .852 & .846  &.904 \\
% DFMNet$_{21}$ (\citeauthor{Zhang2021DFMNet}) & - & - & .019 & .932 & .938  &.973 & .024 & .912 & .926  &.961 & .039 & .913 & .912  &.950 & .040 & .904 &.908  &.948 & .049 & .890 & .885  &.926 \\%& - & - & -  & - \\
% TriTrans$_{21}$(\citeauthor{}) & & & .014 & .946 & .943  &.978 & .020 & .930 & .928  &.963 & .030 & .934 & .920  &.953 & .033 & .920 & .908  &.949 & .043 & 916 & .886  &.928  \\ %& - & - & -  & - \\
CMINet$_{21}$ (\citeauthor{cascaded_cmi}) & - & - &-&-&-&-&-&-&-&-&.064&.862&.877&.911  \\%& - & - & -  & - \\
DSNet$_{21}$ (\citeauthor{wen2021dynamic}) & 172.4 &141.2&-&-&-&-&.133&.676&.716&.736&.068&.849&.867&.890 \\ 
UTANet$_{21}$ (\citeauthor{zhao2021rgb}) & 48.6& 27.4 &-&-&-&-&-&-&-&-&-&-&-&- \\%& .042 & .881 & .885  &- \\
BIANet$_{21}$ (\citeauthor{zhang2021bilateral}) & 49.6&59.9&-&-&-&-&-&-&-&-&-&-&-&-  \\
SPNet$_{21}$ (\citeauthor{zhou2021specificity})& 150.3&68.1&-&-&-&-&-&-&-&-&-&-&-&- \\ % & .044 & .883 & .871  & .915 \\
\rowcolor{gray!15}VST$_{21}$ (\citeauthor{liu2021visual})& 83.3 & 31.0&.024&.948&.943&.969&.113&.763&.759&.826&.061&.889&.882&.921 \\
\rowcolor{gray!15}RD3D+$_{22}$ (\citeauthor{chen20223})& 28.9 & 43.3&.030&.945&.936&.964&.130&.697&.718&.786&-&-&-&- \\
\rowcolor{gray!15}BPGNet$_{22}$ (\citeauthor{yang2022bi})&84.3&138.6&.031&.938&.930&.958&-&-&-&-&.066&.875&.874&.908 \\
% MobileSal$_{22}$ (\citeauthor{})\\
C2DFNet$_{22}$ (\citeauthor{zhang2022c}) & 47.5&21.0&.025&.934&.931&.958&-&-&-&-&.065&.863&.880&.883\\ 
% 
MVSalNet$_{22}$ (\citeauthor{zhou2022mvsalnet})   & - &-&-&-&-&-&-&-&-&-&.072&.880&.856&.906  \\  
SPSN$_{22}$ (\citeauthor{lee2022spsn})  & 37.0& 100.3&-&-&-&-&-&-&-&-&-&-&-&-    \\   

% RFNet$_{22}$(\citeauthor{}) & 365 & &.015& .946& .941& .977
% &.020&.932&.931&.962
% & .029 & .936 &.926& .951 
% &.035&.921&.911& .944 
% &.042& .916 & .893 &.931 \\

HiDANet$_{23}$~(\citeauthor{wu2023hidanet})&  130.6&71.5&-&-&-&-&-&-&-&-&-&-&-&-  \\

\hline
% \rowcolor[RGB]{235,235,250 
\rowcolor{gray!15}\nMethod{}-T& 5.9 &4.5 &.027&.940&.935&.960&.115&.800&.747&.819&.059&.892&.876&.910  \\
\rowcolor{gray!15}\nMethod{}-S&18.5&10.1&.027&.942&.938&.963&.113&.802&.751&.821&.059&.895&.880&.913\\
\rowcolor{gray!15}\nMethod{}-B&29.3&16.7&.025&.945&.940&.966&.109&.809&.755&.823&.058&.899&.881&.920\\
\rowcolor{gray!15}\nMethod{}-L&38.8&26.2&\highlight{.023}&\highlight{.952}&\highlight{.945}&\highlight{.970}&\highlight{.106}&\highlight{.813}&\highlight{.760}&\highlight{.826}&\highlight{.056}&\highlight{.903}&\highlight{.885}&\highlight{.925}\\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{center}
\end{table}
